Towards Zero-trust Security for the Metaverse

By focusing on immersive interaction among users, the burgeoning Metaverse can be viewed as a natural extension of existing social media. Similar to traditional online social networks, there are numerous security and privacy issues in the Metaverse (e.g., attacks on user authentication and impersonation). In this paper, we develop a holistic research agenda for zero-trust user authentication in social virtual reality (VR), an early prototype of the Metaverse. Our proposed research includes four concrete steps: investigating biometrics-based authentication that is suitable for continuously authenticating VR users, leveraging federated learning (FL) for protecting user privacy in biometric data, improving the accuracy of continuous VR authentication with multimodal data, and boosting the usability of zero-trust security with adaptive VR authentication. Our preliminary study demonstrates that conventional FL algorithms are not well suited for biometrics-based authentication of VR users, leading to an accuracy of less than 10%. We discuss the root cause of this problem, the associated open challenges, and several future directions for realizing our research vision.

==> 00.abstract.tex <==
Metaverse, with the combination of the prefix ``meta'' (meaning transcending) and the word ``universe'', has been deemed as the next-generation (NextG) Internet.
%
While there is no consensus on the definition, a narrow depiction of Metaverse is a universal virtual world focusing on social interaction, which connects multiple 3D virtual environments via the Internet.
%(\ie a network of virtual worlds).
%
Similar to online social networks, in the Metaverse, there will be security and privacy issues, such as attacks on user authentication and impersonation. 
%
Moreover, there will be new types of challenges, for example, securing the non-fungible token (NFT), which involves the physical world when users buy and trade assets. 
%
%Moreover, online harassment can be exacerbated in the immersive environment of Metaverse by features including free avatar movements and enhanced feelings of presence and embodiment.
%
Although security and privacy are usually an afterthought in systems research, we should take them into consideration from day one when designing and implementing the Metaverse.
%
In this project, we aim to explore the emerging security threats and privacy concerns in social virtual reality (VR) platforms, the early prototype of the burgeoning Metaverse, and propose novel schemes to defend security attacks and preserve sensitive user information.
%
We propose to leverage privacy-preserving machine learning (ML) approach -- federated learning (FL) to implement continuous authentication towards users in social VR platforms. 

==> 06.related.tex <==
\noindent {\bf Security in VR.}
While VR could bring users an immersive experience in a virtual world, it leads to a host of security issues.
%
%Yarramreddy~\etal~\cite{yarramreddy2018forensic} analyzed how user assets in social VR, such as user accounts and UGC, are stored in the client and the server, and discussed the potential attack methods.
%
Casey~\etal~\cite{casey2019immersive} implemented several attacks on users' controllers, causing them to feel uncomfortable and even motion sickness.
%
Valluripally~\etal~\cite{valluripally2021modeling} used attack-fault trees to study the impact of different attack methods on the user experience of social VR.
%
% model security and privacy issues in social VR to study the impact of different attack methods on user experience~\cite{valluripally2021modeling,valluripally2020attack}.
%
%Adams~\etal~\cite{adams2018ethics} conducted a study on VR users and developers to establish a foundational understanding of security and privacy issues in VR.
%
In this work, we focus on  VR authentication, an essential security issue in the Metaverse.

%another type of security issue in VR -- user authentication.


% \vspace{0.05in}
% \noindent {\bf Security in AR/MR.}

\vspace{0.05in}
\noindent {\bf Biometrics-based Authentication in VR.}
There is a plethora of work on biometrics-based authentication in VR~\cite{zhu2020blinkey,miller2021using,zhang2017continuous}.
% from different perspectives~\cite{zhu2020blinkey,miller2021using,zhang2017continuous}.
%
Miller \etal~\cite{miller2021using} designed a specific task (\ie throwing a ball) for authenticating users,
%
%But these methods are 
which is intrusive and not suitable for continuous authentication.
%
Zhang \etal~\cite{zhang2017continuous} %To employ biometric data,
proposed non-intrusive implicit stimuli in the VR for authentication. %is a potential approach.
%existing work designed non-intrusive implicit stimuli in the VR scene and then collected the users' head and gaze movements for continuous authentication~\cite{zhang2017continuous}.
%
%In addition to behavioral biometrics data, physiological biometrics from users, such as pupil, can be used in VR authentication~\cite{zhu2020blinkey}.
%and extraocular muscles
%
However, %the servers of 
the above work required raw data directly from users to train the models, which may compromise their privacy.
%
In contrast, we aim to design a VR authentication system without leaking users' privacy by leveraging FL.
%\bo{trim this paragraph.}


\vspace{0.05in}
\noindent {\bf Continuous Authentication}, as a powerful means of protecting users, has been extensively studied on different types of mobile devices.
%
% There are some works exploring continuous authentication methods on different types of mobile devices.
%
%Touchalytics~\cite{frank2012touchalytics} utilizes the user's interaction with the smartphone's touch screen to perform continuous authentication.
%
VAuth~\cite{feng2017continuous} provided a continuous verification solution for voice assistants on wearable devices by matching vibration signals with voice signals.
%
Trueheart~\cite{zhao2020trueheart} benefited from the user's pulsation signal collected by the photoplethysmograph sensor in wristband wearables to conduct continuous authentication.
%
Different from the above work, in this paper, we focus on the continuous authentication approach on another type of mobile device, VR headsets.

\iffalse
\vspace{0.05in}
\noindent {\bf Client Selection in FL.} Client selection has emerged as an indispensable problem in FL since it can
improve training efficiency, reduce communication overhead, and potentially address the scalability issue of FL~\cite{wang2021field}.
%
Unlike traditional client selection strategies, such as random selection that has been widely used, newly proposed client selection algorithms focus on selecting clients with suitable data and available resources for training, and use the client state information to guide the selection~\cite{cho2020client}.
%
ClusterFL~\cite{ouyang2021clusterfl} utilizes the cluster structure among clients based on their data distribution.
%
It drops the clients that converge slowly or are not directly related to others, reducing the communication time.
%
Oort~\cite{lai2021oort} leverages both the system and data heterogeneity to select the clients.
%
It prioritizes clients who have data that provides the most excellent utility in improving model accuracy and the ability to run training.
%
PyramidFL~\cite{li2022pyramidfl} first identifies suitable clients from the server perspective, then uses the proposed utilization algorithm locally for further client selection.
%
However, the existing client selection algorithm cannot be directly applied to \name.
%
As we discussed in \S\ref{sec:boosting}, we need to guarantee \name has high authentication accuracy for every user.
%
Therefore, we need to involve all clients in training and cannot simply discard any of them.
\fi

% \vspace{0.05in}
% \noindent {\bf Federated Learning for User Authentication.}
% FL lets the server and client jointly train a model while protecting user data privacy.
% %
% When leveraging FL to train the user authentication model, a key challenge is that each client holds only positive label data~\cite{hosseini2021federated,yu2020federated}.
% %
% Some works in the face recognition field dedicated to solving this problem~\cite{meng2022improving,aggarwal2021fedface,liu2022fedfr}.
% %
% FedFace~\cite{aggarwal2021fedface} utilizes a pre-trained face feature extractor to initialize client class embeddings.
% %
% FedFR~\cite{liu2022fedfr} utilizes additional data from public datasets to achieve feature space consistency via finetune or distillation.
% %
% PrivacyFace~\cite{meng2022improving} leverages differential privacy (DP) to extract non-sensitive information from clients to mitigate the problem of having only positive labels on the client. 





















\iffalse
BlinKey: A Two-Factor User Authentication Method for Virtual Reality Devices* (IWMUT20 )
https://ranger.uta.edu/~mingli/publications/BlinKey.pdf

Knowledge-driven Biometric Authentication in Virtual Reality (2020 CHI extended)
https://groups.inf.ed.ac.uk/tulips/papers/mathis2020chi2.pdf

A Siamese Neural Network for Behavioral Biometrics Authentication
https://openreview.net/forum?id=MG8Zde0ip6u

\vspace{0.05in}
\noindent {\bf Behavior-based Authentication.}

head+gaze:
Using Gaze Behavior and Head Orientation for Implicit Identification in Virtual Reality * (VRST21)
https://dl.acm.org/doi/10.1145/3489849.3489880

Continuous Authentication Using Eye Movement Response of Implicit Visual Stimuli* (17 IMWUT 22-page)
https://dl.acm.org/doi/10.1145/3161410

RubikAuth: Fast and Secure Authentication in Virtual Reality (CHI EA20)
https://dl.acm.org/doi/abs/10.1145/3334480.3382827

Behavioural Biometrics in VR
Identifying People from Body Motion and Relations in Virtual Reality (CHI2019)
https://dl.acm.org/doi/abs/10.1145/3290605.3300340


\vspace{0.05in}
\noindent {\bf Continuous Authentication.}


Several biometrices-based/ behavior-based continuous authentication work form this group *:

method:  ball-throwing application (gait-based)

https://tars.clarkson.edu/

biometrices-based

Combining Pairwise Feature Matches from Device Trajectories for Biometric Authentication in Virtual Reality Environments
https://tars.clarkson.edu/papers/AIVR2019_Ajit.PDF

Task-Driven Biometric Authentication of Users
in Virtual Reality (VR) Environments
https://tars.clarkson.edu/papers/TaskDriven_MMM2019.PDF

Temporal Effects in Motion Behavior for Virtual Reality (VR) Biometrics (2022 VR full paper)
https://ieeexplore.ieee.org/document/9756745

Combining Real-World Constraints on User Behavior with Deep Neural Networks for Virtual Reality (VR) Biometrics (2022 VR full paper)
https://ieeexplore.ieee.org/document/9756791

behavior-based

Realtime Behavior-Based Continual Authentication of Users in Virtual Reality Environments ( 2019 AIVR 2-page)
https://ieeexplore.ieee.org/abstract/document/8942391

Within-System and Cross-System Behavior-Based Biometric Authentication in Virtual Reality (2020 VRW 6-page)
https://ieeexplore.ieee.org/document/9090572

Using Siamese Neural Networks to Perform Cross-System Behavioral Authentication in Virtual Reality (2021 VR Full Paper)
https://tars.clarkson.edu/papers/VR2021_Miller.PDF

Temporal Effects in Motion Behavior for Virtual Reality (VR) Biometrics (2022 VR full paper)
https://ieeexplore.ieee.org/document/9756745

Combining Real-World Constraints on User Behavior with Deep Neural Networks for Virtual Reality (VR) Biometrics (2022 VR full paper)
https://ieeexplore.ieee.org/document/9756791



Head-Movement:
VRCAuth: Continuous Authentication of Users in Virtual Reality Environment Using Head-Movement (2021 ICCES, 6-page)
https://ieeexplore.ieee.org/document/9137914 

Analysis of head and torso movements for authentication (2018 ISBA 8-page)
https://ieeexplore.ieee.org/document/8311460

gaze: 
Continuous Authentication Using Eye Movement Response of Implicit Visual Stimuli* (17 IMWUT 22-page)
https://dl.acm.org/doi/10.1145/3161410

\rz{FL4auth}

paper repo of FL:

https://github.com/innovation-cat/Awesome-Federated-Machine-Learning 

\url{https://arxiv.org/pdf/2007.04618.pdf}

\url{https://arxiv.org/pdf/2104.07158.pdf}

http://proceedings.mlr.press/v139/hosseini21a/hosseini21a.pdf (ICML '21)

ICLR reject revise: https://openreview.net/forum?id=InGI-IMDL18

speaker verification

https://dingye.me/data/paper/ica3pp21.pdf

https://arxiv.org/pdf/2008.02651.pdf

End-to-end speech recognition from federated acoustic models (ICASSP 2022)
https://arxiv.org/pdf/2104.14297.pdf
https://github.com/yan-gao-GY/Flower-SpeechBrain

FedSTAR: Federated Self-Training for Semi-Supervised Audio Recognition* (ACM Trans. Embedd. Comput. Syst 2022 )
https://ieeexplore.ieee.org/document/9746356 and
https://arxiv.org/pdf/2107.06877.pdf
https://github.com/FederatedML/FedSTAR

face recognition 

https://arxiv.org/pdf/2201.12467.pdf DP

https://arxiv.org/pdf/2112.07246.pdf

https://arxiv.org/pdf/2105.02501v1.pdf

http://biometrics.cse.msu.edu/Publications/Face/IJCB_2021_FaceFL_Final.pdf*
https://github.com/illidanlab/fedface


FedFR: Joint Optimization Federated Framework for Generic and Personalized
Face Recognition*
https://www.aaai.org/AAAI22Papers/AAAI-11407.LiuCT.pdf
https://github.com/jackie840129/FedFR


Federated Learning from Only Unlabeled Data with Class-conditional-sharing Clients
https://openreview.net/pdf?id=WHA8009laxu

Horizontal Federated Learning; Android

Communication-Efficient Learning of Deep Networks from Decentralized Data

https://arxiv.org/abs/1602.05629

https://github.com/vaseline555/Federated-Averaging-PyTorch

Behavioral Biometrics for Continuous Authentication in the Internet-of-Things Era: An Artificial Intelligence Perspective
https://ieeexplore.ieee.org/document/9121981
\fi

